Your representations are in the network: composable and parallel adaptation for large scale models

We propose InCA, a lightweight method for transfer learning that cross-attends to any activation layer of a pre-trained model. During training, InCA uses a single forward pass to extract multiple activations, which are passed to external cross-attention adapters, trained anew and combined or selected for downstream tasks. We show that, even when selecting a single top-scoring adapter, InCA achieves performance comparable to full fine-tuning, at a cost comparable to fine-tuning just the last layer. For example, with a cross-attention probe 1.3% the size of a pre-trained ViT-L/16 model, we achieve performance within 0.2% of the full fine-tuning paragon at a computational training cost of 51% of the baseline, on average across 11 downstream classification. Unlike other forms of efficient adaptation, InCA does not require backpropagating through the pre-trained model, thus leaving its execution unaltered at both training and inference. The versatility of InCA is best illustrated in fine-grained tasks, which may require accessing information absent in the last layer but accessible in intermediate layer activations. Since the backbone is fixed, InCA allows parallel ensembling as well as parallel execution of multiple tasks. InCA achieves state-of-the-art performance in the ImageNet-to-Sketch multi-task benchmark.

==> commands_and_packages.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THEOREMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \theoremstyle{plain}
%\newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{proof}[theorem]{Proof}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{corollary}[theorem]{Corollary}
% \theoremstyle{definition}
%\newtheorem{assumption}[theorem]{Assumption}
% \theoremstyle{remark}
%\newtheorem{remark}[theorem]{Remark}

% \usepackage{xspace}
% \newcommand*{\eg}{e.g.\@\xspace}
% \newcommand*{\ie}{i.e.\@\xspace}
% \newcommand*{\iid}{i.i.d.\@\xspace}
% \newcommand*{\wrt}{w.r.t.\@\xspace}
% \newcommand*{\wlogg}{w.l.o.g.\@\xspace}

\usepackage{xcolor}

\newcommand{\real}{\mathbb{R}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\newcommand{\feats}{g}
\newcommand{\model}{f}
\newcommand{\adapter}{{f^*}}
\newcommand{\numtokens}{p}
\newcommand{\featsdim}{d}
\newcommand{\numclasses}{C}
\newcommand{\numlayers}{n}
\newcommand{\mixcoeff}{b}
\newcommand{\params}{W}
\newcommand{\numsamples}{N}
